Reward-guided Fine-Tuning of One-Step Generative Models via Wasserstein Gradient Flow

To mitigate the time complexity of generative models, one-step generative models have recently emerged through direct mapping from noise to data in a single forward pass. However, the reward-guided fine-tuning method of one-step generative models remains largely unexplored. To address this, we consider one-step generators from an optimal transport view, investigating Wasserstein Gradient Flow (WGF) for modeling smooth and controlled distributional evolution in probability space. We then propose a novel reward-guided fine-tuning of a one-step generative model via WGF. We derive a practical training method that requires no reward gradients, thereby handling both non-differentiable and differentiable rewards. Moreover, our method provides smooth and stable reward-guided distributional updates while mitigating reward hacking and mode collapse. Experiments on 2D synthetic data, CIFAR-10, and ImageNet 256$\times$256 with diverse rewards, including JPEG (in)compressibility, class probability, Black-and-White and CLIP alignment, show that our method achieves better reward alignment compared to baselines.

==> text.tex <==
\section{Introduction}
Diffusion models \citep{song2021scorebased, ho2020denoising} have emerged as the leading paradigm for data generation, achieving high-quality image synthesis. However, their widespread use is heavily bottlenecked by slow inference speeds due to their iterative denoising steps. To address this computational limitation, recent research has focused on one-step generative frameworks, such as consistency models or flow maps \cite{consistency, song2024improved, lu2025simplifying, kim2023consistency, MeanFlow, frans2025one}. 
By directly mapping from the noise distribution to the data distribution in a single forward pass, these models are efficient while preserving quality.

Recent advances in fine-tuning have demonstrated remarkable success across diverse tasks, including image aesthetics \cite{DDPO, clark2024directly, prabhudesai2023aligning}, image compression \cite{DPOK, DDPO} and text-image alignment \cite{DDPO, clark2024directly}. An especially promising framework is performing reward fine-tuning in the one or few step frameworks, where the model generates samples in a single forward pass to reduce computational cost. Therefore, recent studies \citep{shekhar2025rocm, jia2025reward, oertell2024rl} have increasingly highlighted the importance of fine-tuning in the one or few step frameworks.
%At a high level, these works share the common goal of jointly achieving fast inference and reward maximization, typically through distillation frameworks or few step MDP formulations.

Despite this growing interest in fast inference, it is difficult to apply existing fine-tuning methods for the multi-step diffusion models \cite{DDPO, DPOK} into one step generation. Without intermediate steps, these fine-tuning methods cannot be applied due to their non-linear trajectory, where a fundamental gap arises from the fact that diffusion-based fine-tuning models require iterative denoising steps. 
In contrast, one-step models generally focus on a linear generation path \cite{uotm}.
% Therefore, existing diffusion based fine-tuning frameworks can not be directly applied to one-step generative models. 

To address this gap, we propose a novel fine-tuning method of one-step generative model via \textbf{Wasserstein Gradient Flow (WGF)}. 
WGF provides a suitable framework for fine-tuning method of one-step generative model by smooth and controlled distributional dynamics in Wasserstein space \cite{ambrosio}. In contrast to diffusion-based fine-tuning framework that rely on stochastic multi-step trajectories, WGF directly optimizes the evolution of the model distribution in probability space. As a result, a fine-tuning method via WGF enables stable distributional updates without requiring iterative inference. 
{Moreover, by operating in Wasserstein space, the model evolves through conservative modifications around the pretrained distribution, effectively mitigating reward hacking and mode collapse.}
% Moreover, the model evolves through small and conservative modifications around the pretrained distribution by Wasserstein space. Therefore, fine-tuning via WGF mitigates reward hacking and mode collapse while preserving stable optimization.

% By this motivation, we propose a novel reward-guided fine-tuning of one-step generative model via Wasserstein Gradient Flow (WGF). And we propose our adversarial learning objective by semi-dual JKO and fine-tuning parameterization . 
We formulate reward-guided fine-tuning as a WGF problem that evolves the pretrained distribution toward a reward-weighted target. To make this tractable, we discretize the continuous WGF using the JKO scheme and derive a practical adversarial learning objective via semi-dual formulation \cite{choi2024scalable} and importance sampling. Our contributions are summarized as follows:
\begin{itemize}[leftmargin=*, topsep=-1pt, itemsep=-1pt]
    \item We present the first framework for reward-guided fine-tuning of one-step generative models based on the mathematical frameworks of WGF and optimal transport.
    \item We derive a practice training algorithm via the JKO scheme and importance sampling that handles both differentiable and non-differentiable rewards.
    \item Experiments demonstrate that our method achieves superior performance compared to baselines across both differentiable and non-differentiable reward functions.
\end{itemize}

% \blue{Our primary contribution is to formulate reward-guided fine-tuning as WGF problem, offering a new mathematical perspective on generative model fine-tuning. Additionally, our method is naturally interpreted an online learning algorithm by the importance sampling and directly handles both differentiable and non-differentiable rewards. Empirically, we evaluate our proposed method on both 2D synthetic distributions and high-dimensional image benchmark CIFAR-10 \cite{Krizhevsky2009LearningML}. Extensive experiments demonstrate that reward-guided fine-tuning baselines frequently suffer from severe mode collapse in one-step generation. However, our method successfully across both differentiable and strictly non-differentiable constraints (e.g., JPEG compressibility) without compromising the structural fidelity of the pretrained distribution.
% }


\section{Preliminaries}

\paragraph{Notations and Assumptions}
Let $\mathcal{P}(\mathbb{R}^d)$ be the set of probability distributions on $\mathbb{R}^d$ that are absolutely continuous with respect to the Lebesgue measure. For a measurable map $T$, $T_\# \mu$ represents the pushforward distribution of $\mu$. 
The 2-Wasserstein distance $\mathcal{W}_2 (\cdot, \cdot)$ is defined as follows:
\begin{equation} \label{eq:2-was}
    \mathcal{W}_2 (\rho, \xi) := \left(\min_{\pi \in \Pi(\rho, \xi)} \int_{\mathbb{R}^d \times \mathbb{R}^d} \lVert x-y \rVert_2^2 d\pi(x,y)\right)^{\frac{1}{2}},
\end{equation}
where $\Pi(\rho, \xi)$ denotes the set of joint probability distributions on $\mathbb{R}^d\times\mathbb{R}^d$ whose marginals are $\rho$ and $\xi$. 
Moreover, $f^*$ indicates the convex conjugate of a function $f$, i.e., $f^{*}(y) = \sup_{x \in \mathbb{R}}\{\langle x, y \rangle - f(x)\}$ for $f:\mathbb{R}\rightarrow [-\infty, \infty]$.

\subsection{One-Step Generative Models}

% Diffusion models and flow matching corresponds to continuous-time generative models that learn a continuous transformation from a tractable noise distribution $p_0$ to the target data distribution $p_1 = p_{\text{data}}$. 
Diffusion models \citep{song2021scorebased} and flow matching \citep{lipman2023flow,liu2022flow} learn a continuous transformation from a tractable noise distribution $p_0$ to the target data distribution $p_1 = p_{\text{data}}$.
This continuous transformation is represented by modeling the probability flow via Ordinary Differential Equation (ODE) as follows: 
\begin{equation} \label{eq:pf_ode}
\mathrm{d}x_t = v_\theta(x_t, t) \mathrm{d}t, \quad t \in [0, 1],
\end{equation}
where $v_{\theta}$ denotes a velocity field over a continuous timestep $t \in [0,1]$. In diffusion models, $v_{\theta}$ is implicitly defined via the score function (PF-ODE) \citep{song2021scorebased}, while in flow matching it is trained through a direct regression to the ground-truth conditional vector field \citep{lipman2023flow,liu2022flow}. To generate a new sample, the probability flow ODE (PF-ODE) $v_{\theta}$ is solved from $t =0 $ to $t =1$, starting with an initial value $z \sim \mathcal{N}(0,I)$. 

Since solving this ODE over $t \in [0,1]$ requires numerical integration, the resulting iterative procedure involves tens to hundreds of neural network evaluations, leading to computationally expensive inference. To enable one-step or few-step efficient generation by directly learning the solution to the probability flow (Eq. \ref{eq:pf_ode}), recent models like Consistency Trajectory Model (CTM) \cite{kim2023consistency} and MeanFlow \cite{geng2025mean} distill or parameterize the flow map, which maps a state at time $t$ directly to time $s$:
\begin{equation}
    \psi(x_t, t, s) = x_t + \int_{t}^{s} v_\theta(x_\tau, \tau) \mathrm{d}\tau.
\end{equation}
By directly learning this mapping, the entire generation process can be executed in a single forward pass: 
\begin{equation}
    x_1 = \psi(x_0, 0, 1) = G_\theta(x_0).
\end{equation}
In this work, we assume access to a pretrained one-step generative model $T_0 : \mathbb{R}^d \to \mathbb{R}^d$ such that $(T_0)_\#\mu \approx \nu$, where $\mu$ is a Gaussian prior and $\nu$ is the data distribution.

\subsection{Wasserstein Gradient Flow and JKO scheme}

\paragraph{Wasserstein Gradient Flow} 
Given a functional $\mathcal{F}(\rho)$ on $\rho\in \mathcal{P}(\mathbb{R}^d)$, the Wasserstein Gradient Flow (WGF) \cite{ambrosio} describes the dynamics of probability density $\{\rho_{t}\}_{t \geq 0}$, following the steepest descent direction of $\mathcal{F}(\rho)$. Here, the metric on $\mathcal{P}(\mathbb{R}^d)$ is defined as the 2-Wasserstein distance $\mathcal{W}_2$ (Eq \ref{eq:2-was}). 
The WGF can be explicitly written by the PDE as follows:
\begin{equation} \label{eq:WGF}
    \frac{\partial \rho}{\partial t} = \nabla \cdot \left( \rho \nabla \frac{\delta \mathcal{F}}{\delta \rho} \right),
\end{equation}
where $\frac{\delta\mathcal{F}}{\delta \rho} $ denotes the first variation of $\mathcal{F}$ with respect to standard $L_2$ metric \cite{villani}.

When $\mathcal{F}(\rho)$ is given as the $f$-divergence $D_f$ with respect to the target distribution $\nu$, \textbf{WGF describes the trajectories of probability density $\{\rho_{t}\}_{t \geq 0}$ evolving from $\mu=\rho_{0}$ towards $\nu$} by minimizing $\mathcal{F}(\rho)$:
\begin{equation} \label{eq:f-div}
    \mathcal{F}(\rho) := D_f (\rho | \nu) = \int f \left( \frac{d \rho}{d \nu} \right) d \nu.
\end{equation}
In our setting, $\rho_0$ = pre-trained model distribution. $\nu$ reward tilted distribution.

\paragraph{JKO scheme}
Computing the continuous WGF is a challenging problem. To address this, \citet{jko} proposed a time discretization scheme to approximate WGF, called the \textbf{JKO scheme}. In this scheme, when given the current JKO step $\mu_{k}$, the next JKO step $\mu_{k+1}$ is formally defined as follows:
\begin{equation} \label{eq:jko}
    \mu_{k+1} = \underset{\rho \in \mathcal{P}(\mathbb{R}^d)}{\text{argmin}} \left[ \frac{1}{2h} \mathcal{W}_2^2 (\rho, \, \mu_{k}) + \mathcal{F}(\rho) \right].
\end{equation}
where $\mu_{0}=\mu$ is the initial condition. Intuitively, $h$ can be understood as the step size of time discretization. As $h \to 0$, the sequence $\{\mu_k\}$ converges to the continuous WGF trajectory $\{\rho_{kh}\}$.




\section{Method}
In this section, we propose a novel framework for reward-guided fine-tuning of one-step generative models via Wasserstein Gradient Flow (WGF). In \cref{sec:formulation}, we formulate reward-guided fine-tuning as a WGF problem, describing the dynamics from the pretrained distribution $\nu$ to the reward-weighted target $\nu_r$. In \cref{sec:jko_reformulation}, we discretize these continuous dynamics by the JKO scheme and reformulate each JKO step via its semi-dual form. In \cref{sec:algorithm}, we introduce our algorithm and implementation details. 

\subsection{Problem Formulation} \label{sec:formulation}
Our goal is to fine-tune a one-step generative model $T_0$ to generate samples from a reward-weighted distribution $\nu_{r}$. Let $T_0: \mathbb{R}^{d} \to \mathbb{R}^{d}$ be a pretrained one-step generative model trained on an (uncontrolled) data distribution $\nu$ with a (Gaussian) prior distribution $\mu = \mathcal{N}(0, I)$, such that $(T_0)_{\#} \mu \approx \nu$. Here, the reward-weighted distribution is defined as 
\begin{multline} \label{eq:reward_weighted_target}
    \nu_{r} (y) = \frac{\exp \left(\beta \cdot r(y) \right)}{M} \nu(y) \\
    \text{where} \quad M_{\beta} = \int \exp( \beta \cdot r(y) ) d\nu(y).
\end{multline}
where $M_\beta$ denotes the normalizing constant and $\beta >0$ is a reward intensity parameter controlling the trade-off between data distribution and reward. Here, $r: \mathbb{R}^{d} \to \mathbb{R}$ is a given off-the-shelf reward function (e.g., aesthetic score \cite{schuhmann2022laion}, compression ratio, classifier output), which may be non-differentiable.
Moreover, we do not have direct access to samples from $\nu_r$. 

We formulate fine-tuning as minimizing the $f$-divergence between the model distribution and the reward-weighted target via WGF. Specifically, we define the energy functional:
\begin{equation} \label{eq:wgf_finetuning}
\mathcal{F}_r (\rho) = D_f(\rho \| \nu_r) \quad \text{for } \rho \in \mathcal{P}(\mathbb{R}^d),
\end{equation}
which measures the divergence between the current distribution and the reward-weighted target $\nu_r$. The WGF $\{ \rho_{t} \}_{t \geq 0}$ starting from $\rho_0 = (T_0)_\#\mu$ describes the evolution of probability density from pretrained model to $\nu_r$ by following the steepest descent of $F_r(\rho)$ in the Wasserstein space $\mathcal{W}_2$. 
\begin{equation} \label{eq:WGF in fine-tuning}
\frac{\partial \rho}{\partial t} = \nabla \cdot \left(\rho \nabla \frac{\delta \mathcal{F}_r}{\delta \rho}\right), \quad \rho_0 = (T_0)_\#\mu.
\end{equation} 

\paragraph{Convergence guarantees}
We establish theoretical convergence guarantees for our fine-tuning via WGF based on \citep[Thm. 11.2.1]{ambrosio}. In practice, we obtain exponential convergence rates under stronger regularity conditions. Suppose $\nu_r$ is $\lambda$-strongly log-concave. Then, under KL divergence as the $f$-divergence, $D_{KL}(\cdot \| \nu_{r})$ achieves exponential convergence in $\mathcal{W}_{2}$-distance as follows:
\begin{equation} \label{eq:exp convergence}
W_2(\rho_t, \nu_r) \leq C \cdot e^{-\lambda t}
\end{equation} 
for some constant $C>0$.

% When $\nu_r$ is a log-concave distribution and generator function of $f$ is a proper, lower semi-continuous, and convex function, the solution $\rho_t$ converges to $\nu_r$.

% \jw{Convergence guarantee statement: \citep[Thm. 11.2.1]{ambrosio} if $\nu_{r}$ is log-cacave and the generator function of $f$ is nice (proper, lower semi-continuous, convex + something). For example, if $\nu_{r}$ is $\lambda$-strongly convex, then $D_{KL}( \rho\| \nu_{r})$ achieves exponential convergence in $W_{2}$-distance.
% } \hs{완료: our case에서 exp convergence guarantee 제시}

\paragraph{Why WGF for fine-tuning?} 
{WGF provides a principled framework for fine-tuning by modeling the evolution of probability distributions along the steepest descent direction of an energy functional in Wasserstein space. This geometric perspective offers several key advantages. First, the steepest descent property induces smooth and controlled distributional updates, as the model evolves gradually toward the reward-weighted target (Figure~\ref{fig:2d_8gaussian}). 
Second, the Wasserstein metric naturally regularizes the distribution shift, ensuring conservative modifications around the pretrained distribution. This minimizing movement structure has been shown to enable stable and efficient optimization in generative modeling and sampling tasks \citep{asbs, asbm}, making WGF particularly suitable for fine-tuning one-step generators without requiring iterative inference steps.}

% This formulation offers several advantages over fine-tuning method. WGF investigates the minimizing dynamics of probability density following the steepest descent direction in Wasserstein space with respect to a given energy functional. 
% This steepest descent property induces the smooth and controlled distributional updates throughout the fine-tuning process (Figure~\ref{fig:2d_8gaussian}). This minimizing movement property have been shown to provide efficient and stable training \citep{asbs, asbm}.

% By leveraging the space of probability distribution space, WGF naturally induces smooth and controlled distributional updates enabling stable optimization throughout the fine-tuning process \citep{asbs, asbm}.\hs{figure ? 2D}
% \jw{steepest descent (or optimal transport)가 좋다의 reference \citep{asbs, asbm}} 


% Controlled deviation from pretrained model

% \hs{JKO part(sec 3.2, semi-dual jko)로 이동}

% % Specifically, WGF explicitly regularizes large distribution shifts during fine-tuning. Since each update is regularized through the Wasserstein distance, the model evolves through small and conservative modifications around the pre-trained distribution. In other words, WGF encourages the model distribution to progressively move toward the reward-weighted target distribution while remaining close to the pre-trained data distribution. Therefore, WGF for fin-tuning mitigates reward hacking and mode collapse while maintaining stable optimization.

% Natural Online learning interpretation (Gradual annealing) 


\subsection{Fine-tuning via JKO Scheme} \label{sec:jko_reformulation}
Computing this continuous WGF in \cref{eq:wgf_finetuning} is a challenging problem. We address this problem via the JKO scheme \citep{jko}, which is a time-discretization scheme to approximate WGF. Under the JKO scheme, the JKO scheme conducts the following iterative update:
\begin{equation} \label{eq:jko_finetuning}
\begin{aligned}
\nu_{k+1} 
&= \underset{\rho \in \mathcal{P}(\mathbb{R}^d)}{\mathrm{argmin}} 
\; \underbrace{
\frac{1}{2h} \mathcal{W}_2^2 (\nu_{k}, \rho) 
+ D_f (\rho \mid \nu_{r})
}_{\mathcal{L}_{\rho}} \\
&\quad \text{with} \quad 
\nu_{0} = T^{\theta}_{\#} \mu \approx \nu.
\end{aligned}
\end{equation}
Note that $h>0$ indicates the step size in the time-discretization. The JKO scheme balances two objectives: the Wasserstein distance term $W_2^2(\rho, \nu_k)$ ensures that the updated distribution stays close to the previous step $\nu_{k}$, while the divergence functional $D_f (\rho \mid \nu_{r})$ leads the distribution toward the reward-weighted target. As the step size $h \to 0$, the JKO step $\{\nu_k\}$ converges to the continuous WGF trajectory $\{\rho_{kh}\}$.

\paragraph{Semi-dual form of JKO}
Following \citet{s-jko}, this JKO step admits a semi-dual formulation. By leveraging the equivalence with the Unbalanced Optimal Transport (UOT) problem \citep{uot1, uot2}, this semi-dual formulation is derived as follows:
\begin{equation} \label{eq:semi-dual-jko}
    \sup_{v \in \mathcal{C}} \int v^c(x) d\nu_k(x) + \int f^\circ(v(y)) d\nu_{r}(y).
\end{equation}
where $v: \mathbb{R}^d \to \mathbb{R}$ is a potential function, $v^c(x) := \inf_y ( c_h(x,y) - v(y) )$ is its $c$-transform with $c_h(x,y) = \frac{1}{2h}\|x-y\|_2^2$, and $f^\circ(x) := -f^*(-x)$ with $f^*$ being the convex conjugate of $f$. 

Here, we implicitly represent the evolving transport map from the $k$-th JKO step $\nu_{k}$ to $(k+1)$-th JKO step $\nu_{k+1}$ via $c$-transform parameterization \citep{otm, fanTMLR}:
\begin{equation}
    \Delta T_{k} : x \mapsto \underset{y}{\arg\min} \left( c(x,y) - v(y) \right).
\end{equation}
Then, $\Delta T_{k}$ satisfies the following:
\begin{equation}
    v^c(x) := c(x,\Delta T_{k}(x)) - v(\Delta T_{k}(x)).
\end{equation} 
Substituting this into Eq.~\eqref{eq:semi-dual-jko} yields the max-min objective for a single JKO step as follows:
\begin{equation} \label{eq:semi-dual-jko-with-transport}
\begin{aligned}
\sup_{v \in \mathcal{C}} \; & \int \inf_{\Delta T_{k}} 
\left[ 
c\left(x, \Delta T_{k}(x)\right) - v(\Delta T_{k}(x)) 
\right] d\nu_k(x) \\
&+ \int f^\circ(v(y)) d\nu_{r}(y).
\end{aligned}
\end{equation}
Importantly, this objective for a single JKO step is equivalent to Source-fixed-UOTM between $\nu_k$ and $\nu_{k+1} = (\Delta T_k)_{\# \nu_k}$ \citet{s-jko}. This equivalence enables our fine-tuning method to leverage the theoretical foundations of optimal transport. Additionally, in adversarial learning perspective, we can interpret $\Delta T_k$ as a \textit{Generator} that maps $\nu_k$ to $\nu_{k+1}$. And potential function $v$ is interpreted as \textit{Discriminator} between $\nu_k$ and $\nu_{k+1}$.

Moreover, since the JKO step inherits 2-Wasserstein cost, the JKO explicitly regularizes large distribution shifts during the fine-tuning process. In practice, the model evolves through small and conservative modifications around the pre-trained distribution. In other words, the JKO scheme encourages the model distribution to progressively move toward the reward-weighted target distribution while remaining close to the pretrained data distribution. Therefore, fine-tuning via the JKO scheme mitigates reward hacking and mode collapse while maintaining stable optimization.

\paragraph{Fine-tuning parameterization}
In our WGF formulation of fine-tuning, the initial distribution $\rho_{0} = \nu_0$ is the pre-trained one-step generative model and this WGF gradually converges to the reward-weighted target distribution $\nu_{r}$. In this respect, $\Delta T_k$ (\cref{eq:semi-dual-jko-with-transport}) can be interpreted as a refinement mapping that progressively transforms the un-controlled distribtuion $\nu_0 \approx \nu$ (\textit{Source distribution}) into $\nu_r$. Let $T_k:\mathbb{R}^d \to \mathbb{R}^d$ denote the cumulative transformation after $k$ refinement steps:
\begin{equation}
    T_k = \Delta T_{k}  \circ \cdots \circ \Delta T_{1} \circ \Delta T_{0}.
\end{equation}
Then, $T_k$ satisfies $T_{k} := \Delta T_{k} \circ T_{k-1}$ and $(T_k)_\# \mu = \mu_{k+1}$. Here, $T_k$ represents our \textbf{fine-tuned generative model} after the $k$-th JKO step. 
Substituting this reparameterization into Eq. \ref{eq:semi-dual-jko-with-transport}, yields the following objective for the $k$-th step:
\begin{equation} \label{eq:reparametrize}
\begin{aligned}
\mathcal{L}_{k} 
= \sup_{v \in \mathcal{C}} \; 
& \int \inf_{T_{k}} 
\Big[
c\big(T_{k-1}(x), T_k(x)\big) - v(T_k(x))
\Big] d\mu(x) \\
&+ \int f^\circ(v(y)) d\nu_{r}(y).
\end{aligned}
\end{equation}

\paragraph{Importance sampling for reward-weighted targets}
The objective in \cref{eq:reparametrize} requires samples from $\nu_{r}$, which are not directly accessible in our setting. We address this via \textbf{importance sampling} using the definition of $\nu_r$:
\begin{equation} \label{eq:importance_sampling_substitution}
\int f^\circ(v(y)) \, d\nu_{r}(y) 
= \int f^\circ(v(y)) \frac{\exp \left(\beta \cdot r(y) \right)}{M} \, d\nu(y),
\end{equation}
This allows us to estimate the integral using samples from $\nu$ (the pretrained distribution), weighted by the reward function $\exp \left(\beta \cdot r(\cdot) \right)$.

In practice, we use samples from the current model distribution $\nu_k = (T_{k-1})_\#\mu$ as the proposal distribution, since $\nu_k$ gradually evolves from $\nu$ toward $\nu_r$ over the course of training. This yields our final training objective:
\begin{equation} \label{eq:final_objective}
\begin{aligned}
\mathcal{L}_{k} 
= \sup_{v_\phi \in \mathcal{C}} \;
& \int \inf_{T_\theta} 
\Big[
c_h\big(T_{k-1}(x), T_\theta(x)\big) - v_\phi(T_\theta(x))
\Big] d\mu(x) \\
&+ \int f^\circ(v_\phi(y)) \frac{\exp \left(\beta \cdot r(y) \right)}{M} \, d\nu_{k}(y),
\end{aligned}
\end{equation}
where we parameterize the potential function as $v_\phi$ and the transport map as $T_\theta$, respectively. The normalization constant $M$ is estimated using a moving average over mini-batches, which adapts as the distribution shifts toward $\nu_r$.

{This formulation provides several practical advantages. First, the importance sampling strategy naturally leads to an online learning algorithm: at each JKO step $k$, we sample from the current model $T_{k-1}$, evaluate rewards, update $M$, and train $(v_\phi, T_\theta)$ using Eq.~\eqref{eq:final_objective}. Second, since our method does not require gradients through the reward function $r(\cdot)$, it directly handles both differentiable and non-differentiable rewards without modification.  Third, while our primary focus is one-step generation, the framework can leverage few-step sampling when generating $y \sim \nu_{k}$ to obtain higher-fidelity samples if computational budget permits.
% Third, for $y$-simulation from $\nu_{k}$, our method is not restricted to the one-step generative models. Hence, the framework can get higher-fidelity samples by leveraging the few-step sampling variants.
}

% This importance sampling strategy naturally leads to an online learning algorithm: at each JKO step $k$, we sample from the current model $T_{k-1}$, evaluate rewards, update $M$, and train $(v_\phi, T_\theta)$ using Eq.~\eqref{eq:final_objective}. The complete procedure is presented in Algorithm~\ref{alg:finetune}.

% \blue{Moreover, since our method does not impose specific assumptions on the pretrained distribution and reward function, it enables highly scalable and broadly applicable across diverse fine-tuning task. Specifically, our method can be applied to arbitrary pretrained distributions, including any one-step and few-step generative models. In addition, our method does not require a differentiable reward function, allowing both differentiable and non-differentiable rewards.}

% \jw{$y$는 Few-step generation 무방, non-differentiable $r$ 가능}
% \jw{\cite{s-jko} 대비 contribution. Problem formulation, unconditional -> importance sample, non-differentiable reward.}


\subsection{Training Algorithm} \label{sec:algorithm}


We now present the complete training procedure for reward-guided fine-tuning via WGF in Algorithm~\ref{alg:finetune}. The algorithm alternates between updating the discriminator (potential function $v_\phi$) and the generator (transport map $T_\theta$), following the adversarial objective in Eq.~\eqref{eq:final_objective}. The training procedure consists of $K$ outer iterations corresponding to JKO steps. Through this iterative process, the fine-tuned generator gradually evolves from the pretrained distribution $\nu$ toward the reward-weighted target $\nu_r$.% (See Figure ?? for the visualization of training dynamics on 2D synthetic datasets).







% In this section, we propose a novel fine-tuning method for one-step generative model via Wasserstein Gradient Flow (WGF). Specifically, we model the dynamics of probability density that evolves from pre-trained one-step generative model distribution to the reward-weighted target distribution $\nu_{r}$ (\cref{sec:formulation},   ). We then reformulate this dynamics by the JKO scheme. Leveraging the equivalence between each JKO step and Neural Unbalanced Optimal Transport, we introduce a new fine-tuning method of one-step generative model via WGF.

% \subsection{Fine-tuning task formulation}
% In this subsection, we formulate fine-tuning task via WGF. Specifically, Our goal is to finetune one-step generative model to generated samples from a reward-weighted distribution. Let $T_0$ be a pretrained one-step generative model trained on an uncontrolled data distribution $\nu$ with a (Gaussian) prior distribution $\mu$, such that $(T_0)_{\#\mu} = \nu$. And the reward-weighted distribution is defined as 
% \begin{equation} \label{eq:reward_weighted_target}
%     \nu_{r} (y) = \frac{r(y)}{M} \nu(y) \quad \text{where} \quad M = \int r(y) d\nu(y).
% \end{equation}
% $M$ denotes the normalizing constant. Here, we assume access only to an off-the-shelf reward function $r(y)$, which may not be differentiable with respect to $y$. Finally, we assume that the pre-trained one-step generative model ($\nu$) is our source distribution and that the reward-weighted distribution ($\nu_r$) is our target distribution for WGF, respectively.

% \subsection{Reformulation of WGF as a UOT problem}
% In this subsection, we define our fine-tuning method via WGF to the JKO scheme and establish equivalence between each JKO scheme and the UOT problem. Here, we begin WGF. We define the energy functional 
% \begin{equation}
% 	\mathcal{F}(\rho) = D_f \left( \rho | \nu_{r} \right) \quad \text{for } \,\, \rho \in W_{2}(\mathbb{R}^{d}).
% \end{equation}
% which measures the divergence between $\rho$ and the reward-weighted target distribution $\nu_r$. Our objective is to evolve the model distribution toward $\nu_r$, by following the Wasserstein gradient flow of $\mathcal{F}(\rho)$, initialized from the pretrained distribution $(T_0)_{\#\mu}$:
% \begin{equation} \label{eq:WGF_ours}
%     \frac{\partial \rho}{\partial t} = \nabla \cdot \left( \rho \nabla \frac{\delta \mathcal{F}}{\delta \rho} \right), \qquad
%     \rho_{0} = (T_{0})_{\#} \mu.
% \end{equation}
% Computing this continuous WGF is a challenging problem. Therefore, we address this problem via the the JKO scheme, which is a time discretization scheme to approximate WGF. Using the JKO scheme, Discretizing this flow yields the following iterative update: 
% \begin{equation} \label{eq:jko-again}
% \begin{aligned}
% \nu_{k+1} 
% &= \underset{\rho \in \mathcal{P}(\mathbb{R}^d)}{\mathrm{argmin}} 
% \; \underbrace{
% \frac{1}{2h} \mathcal{W}_2^2 (\nu_{k}, \rho) 
% + D_f (\rho \mid \nu_{r})
% }_{\mathcal{L}_{\rho}} \\
% &\quad \text{with} \quad 
% \nu_{0} = T^{\theta}_{\#} \mu \approx \nu.
% \end{aligned}
% \end{equation}
% Note that as the step size $h \to 0$, the JKO step $\{\nu_k\}$ converges to the continuous trajectory $\{\rho_{kh}\}$ of the Wasserstein gradient flow. We now reformulate the JKO step as a Unbalanced Optimal Transport \citep{uotm}. Using definition (Eq 1)\hs{Preliminiaries 작성 후 변경}, $\mathcal{}L_{\rho}$ can be written as the follows: 
% \begin{equation}
%     \mathcal{L}_{\rho} =   \min_{\pi \in \Pi(\nu_{k}, \rho)} \int \frac{1}{2h} \lVert x-y \rVert_2^2 d\pi(x,y)  + D_f (\pi_{1} | \nu_{r}).
% \end{equation}
% Note that $\pi_1 = \rho$ in the above equation. Moreover, the UOT problem is a generalization of the classical OT problem. In eq 9 \hs{UOT formulate; Preliminiaries 작성 후 변경, source-fixed UOT 부분을 method 쪽으로, UOT Equation 안 넣어도 흐름 자연스러운듯 ? ; preliminary에서 OT 제외}, if  $\varphi_1$ or $\varphi_2$ is selected to be a convex indicator function $\iota(x) = \begin{cases} 0 & \text{if } x=1, \\  \infty & \text{otherwise} \end{cases}$, then $D_{\varphi}$ takes the following form:
% \begin{equation}
%     D_{\iota}(\pi_{i}|\rho) = 
%     \begin{cases} 
% 		0 & \text{if } \pi_{i} = \rho \,\,\text{ almost-surely.} \\ 
%         \infty & \text{otherwise. }
%      \end{cases}    
% \end{equation}
% In the JKO setting, the problem can be viewed as the UOT problem with $\varphi_1 = \iota$ and $\varphi_2 = f$. Therefore, the WGF is equivalent to the \textbf{Source-fixed UOT} problem via the JKO step. \hs{JKO-step이 Source-fixed UOT인데 WGF 자체가 동일하다 ? + OT preliminary 추가 or 녹이기}

% \subsection{Fine-tuning with Semi-dual Form of JKO step}

% In this subsection, we propose a novel fine-tuning method for solving each JKO step via the Neural Unbalanced Optimal Transport, based on the semi-dual from of the UOT problem. Our model is derived in two steps: (1) By semi-dual form of JKO step, we represent the JKO step as a Adversarial learning object \hs{Neural UOT?} (2) By finetuning parameterization, we represent semi-dual form of JKO step as a Fine-tuning model between pre-trained source distribution and reward-weighted target distribution.

% \paragraph{Semi-dual form of the JKO step}
% In subsection 3.2, We detrive the JKO step to Source-fixed UOT problem. Therefore, we can formulate the semi-dual form of JKO step by the semi-dual form of UOT \citep{uotm} as follow: 
% \begin{equation} 
%     \sup_{v \in \mathcal{C}} \int v^c(x) d\nu_k(x) + \int f^\circ(v(y)) d\nu_{r}(y).
% \end{equation}
% where the $c$-transform of $\nu$ is defined as $v^c(x) := \inf_y ( c(x,y) - v(y) )$. Here, we parametrize $\Delta T_k$ as follows \citep{otm, fanTMLR}: 
% \begin{equation}
%     \Delta T_{k} : x \mapsto \underset{y}{\arg\min} \left( c(x,y) - v(y) \right).
% \end{equation}
% Then, $\Delta T_{k}$ satisfies the following:
% \begin{equation}
%     v^c(x) := c(x,\Delta T_{k}(x)) - v(\Delta T_{k}(x)).
% \end{equation}
% Therefore, the semi-dual form of the JKO step can be formulated as the adversarial learning objective as follows:
% \begin{equation} \label{eq:semi-dual-jko}
% \begin{aligned}
% \sup_{v \in \mathcal{C}} \; & \int \inf_{\Delta T_{k}} 
% \left[ 
% c\left(x, \Delta T_{k}(x)\right) - v(\Delta T_{k}(x)) 
% \right] d\nu_k(x) \\
% &+ \int f^\circ(v(y)) d\nu_{r}(y).
% \end{aligned}
% \end{equation}
% Then this objective for a single JKO step is represented as Source-fixed UOTM \citep{uotm} between $\nu_k$ and $\nu_{k+1} = (\Delta T_k)_{\#\nu_k}$. In adversarial leraning perspective, we can interpret $\Delta T_k$ as a \textit{Generator} that maps $\nu_k$ to $\nu_{k+1}$. And potential function $v$ is interpreted as \textit{Discriminator} between $\nu_k$ and $\nu_{k+1}$.

% \paragraph{Fine-tuning parameterization}
% In section 3.1, we assume that our source distribution is the pre-trained one-step generative model and target distribution is the reward-weighted distribution (Eq 1) \hs{eq problem} in our fine-tuning task. $\Delta T_k$ (eq. ?) \hs{eq problem} represents a refinement mapping that progressively transforms the un-controlled distribtuion $\nu_0 \approx \nu$(\textit{Source distribution}) into the reward-weighted target distribution $\nu_r$. Let $T_k:\mathbb{R}^d \to \mathbb{R}^d$ denote the cumulative transformation after $k$ refinement steps:
% \begin{equation}
%     T_k = \Delta T_{k}  \circ \cdots \circ \Delta T_{1} \circ \Delta T_{0}.
% \end{equation}
% Then, $T_k$ satisfies $T_{k} := \Delta T_{k} \circ T_{k-1}$ and $(T_k)_\# \mu = \mu_{k+1}$. Here, $T_k$ represents our \textbf{fine-tuned generative model} after the $k$-th JKO step. 
% Substituting this reparameterization into Eq. \ref{eq:semi-dual-jko}, yields the following objective for the $k$-th step:
% \begin{equation} \label{eq:reparametrize}
% \begin{aligned}
% \mathcal{L}_{k} 
% = \sup_{v \in \mathcal{C}} \; 
% & \int \inf_{T_{k}} 
% \Big[
% c\big(T_{k-1}(x), T_k(x)\big) - v(T_k(x))
% \Big] d\mu(x) \\
% &+ \int f^\circ(v(y)) d\nu_{r}(y).
% \end{aligned}
% \end{equation}

% \begin{algorithm}[t]
% \caption{Reward-Guided Finetuning via WGF}
% \label{alg:finetune}
%     \begin{algorithmic}[1]
%     % \Require 
%     \REQUIRE Pretrained generator $T_{0}$, discriminator network $v_{\phi}$, reward function $r(\cdot)$, and smoothing rate $\gamma$.
%     \STATE Initialize $T_{\text{old}} \leftarrow T_{0}$, $M \leftarrow 1$
%     \FOR{$k = 0, 1, 2 , \dots, K$}
%         \FOR{$i = 0, 1, 2 , \dots, N$}
%             \STATE Sample mini-batches $z \sim \mathcal{N}(0,I)$
%             \STATE Let $y = T_{\text{old}}(z)$
%             \STATE Compute rewards $\{ r(y) \}$ and update the normalization term:
%             \[
%             M \leftarrow (1 - \gamma) M + \gamma \cdot \text{mean}\{ r(y) \}
%             \]
%             \STATE Generate samples $\hat{y} = T_{\theta}(x)$
%             \STATE \textbf{Discriminator update:} minimize
%             \[
%             \mathcal{L}_{v} = v_{\phi}(\hat{y}) - f^{\circ}\!\left(v_{\phi}(y)\right) \frac{r(y)}{M}
%             \]
%             \STATE Sample $z \sim \mathcal{N}(0,I)$ and compute $\hat{y}_{} = T_{\text{old}}(z)$, $\hat{y} = T_{\theta}(z)$, 
%             \STATE \textbf{Generator update:} minimize
%             \[
%             \mathcal{L}_{T} = c\!\left(\hat{y}, \hat{y}\right) - v_{\phi}(\hat{y})
%             \]
%         \ENDFOR
%         \STATE Update reference generator: $T_{\text{old}} \leftarrow T_{\theta}$
%     \ENDFOR
%     \end{algorithmic}
% \end{algorithm}
% \hs{나중에 알고리즘 위치 수정}

% Note that this reparametrized learning objective $\mathcal{L}_{k}$ corresponds to the $k$-th JKO step. The comprehensive training procedure repeats this step for $k=0, \cdots, K$. 

% Finally, note that for the Monte Carlo estimation of $\mathcal{L}_{k}$, we need samples $y \sim \nu_{r}$, which are not accessible. We address this limitation via \textbf{importance sampling} using Eq. \hs{eq problem}
% \begin{equation} \label{eq:reward_weighted_target}
% \begin{aligned}
% \mathcal{L}_{k} 
% = \sup_{v \in \mathcal{C}} \;
% & \int \inf_{T_k} 
% \Big[
% c\big(T_{k-1}(x), T_k(x)\big) - v(T_k(x))
% \Big] d\mu(x) \\
% &+ \int f^\circ(v(y)) \frac{r(y)}{M} d\nu(y),
% \end{aligned}
% \end{equation}
% \[
% \text{where} \quad M = \int r(y)\, d\nu(y).
% \]

% \hs{뒤에 알고리즘 관한 내용 추가 ? -> M, reward 등 ... }


\section{Related Works}

\paragraph{One-step generative models} 
One-step generative models aim to reduce the inference step in diffusion/flow-based models. Early studies \cite{salimans2022progressive, meng2023distillation} toward this goal focused on distilling pretrained multi-step models into few-step variants. Consistency Models (CM) \cite{song2023consistency} learn a mapping from any point along the ODE trajectory to its endpoint. CM is possible to train one-step models from scratch. Consistency Trajectory Model (CTM) \cite{kim2023consistency} generalize CM by training a neural network to enforce consistency across different time steps. MeanFlow \cite{MeanFlow} learns average velocity field across time intervals. In practice, MeanFlow significantly outperforms other one or few-step diffusion and flow models. In this work, we aim to fine-tune MeanFlow model as one-step generative models. 

\paragraph{Reward Fine-Tuning}
Recent works have explored fine-tuning diffusion and flow models to align with the reward function while preserving the pretrained distribution. An early approach, DDPO \cite{DDPO} directly optimize model parameters for arbitrary rewards but often suffers from reward hacking, where it overfits to a few high-reward samples. To mitigate this, DPOK \cite{DPOK} incorporates KL regularization to preserve diversity. Similarly, ORW-CFM \cite{fan2025online} incorporates the Wasserstein-2 distance to prevent policy collapse and maintain diversity in fine-tuning of flow models. However, since these methods rely on iterative diffusion or flow-based generation processes, they cannot be directly applied to fine-tuning of one-step generative models. 
%Moreover, our method is based on the mathematical foundations of Wasserstein Gradient Flow (WGF) and optimal transport. 
% Therefore, our method provides a novel principled framework for evolving the pretrained model distribution toward the reward weighted target distribution while mitigating reward hacking and mode collapse.

% \js{이 이후는 사실 result라 각 실험에 specific한 setup만 subsection에서 서술하고 (공통적인 건 5.1), 표 제시와 결과 해석 중심 및 우리 장점 중심으로 서술.}
\begin{figure}[t]
    \centering

    \setlength{\fboxsep}{0pt}
    \setlength{\fboxrule}{0.1pt}
    \setlength{\tabcolsep}{0pt}

    \small

    \begin{tabular}{c @{\hspace{3mm}} c}
        \begin{tabular}{c}
            \small Pre-trained \\[1mm]
            \raisebox{-0.5\height}{\fbox{\includegraphics[width=0.20\columnwidth]{figures/8g_pretrained.pdf}}} \\
            \\[-2mm] 
        \end{tabular}
        &
        \begin{tabular}{ccc @{\hspace{2mm}} c}
            \raisebox{-0.5\height}{\fbox{\includegraphics[width=0.20\columnwidth]{figures/iter_05000.pdf}}} &
            \raisebox{-0.5\height}{\fbox{\includegraphics[width=0.20\columnwidth]{figures/iter_15000.pdf}}} &
            \raisebox{-0.5\height}{\fbox{\includegraphics[width=0.20\columnwidth]{figures/iter_25000.pdf}}} & 
            \raisebox{3mm}{\rotatebox{270}{\small Ours}} \\
            \small 5k & \small 15k & \small 25k & \\ [2mm]

            \raisebox{-0.5\height}{\fbox{\includegraphics[width=0.20\columnwidth]{figures/sft_iter_020000.pdf}}} &
            \raisebox{-0.5\height}{\fbox{\includegraphics[width=0.20\columnwidth]{figures/rwr_iter_020000.pdf}}} &
            \raisebox{-0.5\height}{\fbox{\includegraphics[width=0.20\columnwidth]{figures/dpo_iter_020000.pdf}}} & 
            \raisebox{6mm}{\rotatebox{270}{\small Baselines}} \\
            % [0.5mm] \\
            \small SFT & \small RWR & \small DPO & \\
        \end{tabular}

    \end{tabular}

    \caption{\textbf{Qualitative comparison on the 8-Gaussians toy task.} The left panel shows the initial pre-trained gaussian distribution. The top row illustrates the trajectory of our reward-guided fine-tuning method across 5k, 15k, and 25k iterations. In contrast, the bottom row presents the converged results of baselines at 20k steps.}
    \label{fig:2d_8gaussian}
    \vspace{-8pt}
\end{figure}

\section{Experiments}

% The goal of our experiments is to evaluate whether existing reward-based fine-tuning methods can be applied to one-step generative models, and to demonstrate how our approach overcomes their structural limitations. Specifically, we fine-tune a pre-trained MeanFlow model as a one-step generator and compare against standard baselines.
% \jw{Baseline paragraph가 따로 있으니, 굳이 언급 필요없음. Meanflow 모델도 Experimental setting으로}

% \woorim{섹션별 ref 추가하기}
% Our experimental design targets three fundamental questions. In Sec. \ref{sec:2d_synthetic}, (1) Do standard baselines such as SFT, RWR, and DPO remain effective in the one-step setting? (2) Can reward optimization be achieved without sacrificing sample quality in differentiable settings? (3) Does the method generalize to non-differentiable reward functions where gradient-based optimization is not applicable? Through these experiments, we show that existing methods consistently do not provide stable or meaningful improvements in this setting.
% \jw{각 질문에 해당하는 실험 결과를 ref. ex) section 번호 or Table or Fig}

% The primary goal of our experiments is to evaluate the applicability of existing reward-based fine-tuning methods to one-step generative models, and to demonstrate how our proposed approach overcomes their inherent structural limitations. 

% To comprehensively assess our method, we structure our evaluation around three core questions:

{In this section, we evaluate the strength of our method across diverse settings and reward functions.
}

% \begin{itemize}[leftmargin=*, topsep=-1pt, itemsep=-1pt]
%     % \item \textbf{Q1: What are the training dynamics of our one-step generator?} In Section~\ref{sec:2d_synthetic}, evaluating on 2D synthetic data reveals that our method exhibits a gradual and stable training progression, progressively capturing complex multi-modal distributions over time (Figure~\ref{fig:2d_8gaussian}).
    
%     \item In \cref{sec:2d_synthetic}, we visualize training dynamics on 2D synthetic datasets, demonstrating gradual and stable optimization of our WGF formulation.
    
%     % \item \textbf{Q2: Can we optimize strictly non-differentiable rewards?} In Section~\ref{sec:non_diff}, we apply our framework to (in)compressibility tasks. Our approach successfully maximizes the reward without compromising structural integrity, showing a superior reward-FID trade-off.

%     \item In \cref{sec:non_diff}, we evaluate our model on non-differentiable reward functions (compression and incompression).
    
%     % \item \textbf{Q3: Can we maximize rewards without sacrificing fidelity?} In Section~\ref{sec:diff}, we evaluate classification tasks on CIFAR-10. Our method achieves the highest target rewards while effectively avoiding the severe degradation observed in the baselines.

%     \item In \cref{sec:diff}, we evaluate our model on the differentiable reward functions (class probability and brightness). 

%     \item In \cref{sec:ablation_study}, we conduct an ablation study on the reward scale $\beta$ to verify the robust controllability of our method.
% \end{itemize}

% Finally, in Section~\ref{sec:ablation_study}, we conduct an ablation study on the reward scale $\beta$ to verify the robust controllability of our method.

% \subsection{Experimental settings}
% \woorim{consistently fail? 말고 다른 표현으로 수정}

% We evaluate on both a 2D synthetic data and CIFAR-10 \cite{Krizhevsky2009LearningML} to cover low- and high-dimensional settings. Our results show that, while baselines often suffer from instability, mode collapse, or little to no reward improvement, our method achieves stable optimization, effective reward alignment, and robust performance even under non-differentiable reward constraints.

% \woorim{metrics에 대한 설명?} \js{뭐뭐썻다 (ref)는 있어야 하고, full paper에는 간단히 각각 뭐인지설명 }

% \paragraph{Baselines}
% We compare our method with standard fine-tuning approaches commonly used in reward-driven settings, including Supervised Fine-Tuning (SFT), Reward-Weighted Regression (RWR) \cite{peters2007reinforcement}, and Direct Policy Optimization (DPO) \cite{rafailov2023direct}. We have transformed the multi-step rollout \cite{FlowGRPO} into a single MeanFlow step by a single noise injection.
% \jw{인용 추가}

% \woorim{수식 추가하기} \js{수식 부분은 그냥 일단 claude 부탁하고 app으로 내려도 될듯합니다.}
% \begin{itemize}
%     \item \textbf{Supervised Fine-Tuning (SFT)} selects the highest-reward trajectory within each group,
%     \begin{equation*}
%         x^{+} = \arg\max_{x_i} r(x_i),
%     \end{equation*}
%     and optimize the reconstruction objective
%     \begin{equation*}
%         \mathcal{L}_{\text{SFT}} =
%     \end{equation*}
    
%     \item \textbf{Reward-Weighted Regression (RWR)}
%     performs reward-weighted likelihood maximization:
%     \begin{equation*}
%         \mathcal{L}_{\text{RWR}}
%         =
%     \end{equation*}

%     \item \textbf{Direct Preference Optimization (DPO)}
%      optimizes pairwise preferences between higher- and lower-reward samples:
%     \begin{equation*}
%         \mathcal{L}_{\text{DPO}} = 
%     \end{equation*}

% \end{itemize}

% \jw{equation을 통해 설명} 


\subsection{Experimental Settings}


We evaluate our method on both 2D synthetic datasets and CIFAR-10 \cite{Krizhevsky2009LearningML} to cover both low- and high-dimensional settings. We use a pretrained MeanFlow model \citep{MeanFlow} as our one-step generator $T_{0}$.
% While standard baseline approaches frequently struggle with the trade-off between reward maximization and generation stability—often exhibiting severe mode collapse or sub-optimal convergence—our method achieves stable optimization, effective reward alignment, and robust performance even under non-differentiable reward constraints.

% To quantitatively evaluate generation quality and reward alignment, we employ the Fréchet Inception Distance (FID) \cite{heusel2017gans} to measure the fidelity of generated images, and use task-specific metrics, such as JPEG file size, to assess the (in)compressibility objectives.
For quantitative evaluation, we employ the Fréchet Inception Distance (FID) \cite{heusel2017gans} and the task-specific reward functions. FID measures the fidelity of generated images. The task-specific reward functions assess alignment with the target objectives. These two metrics typically exhibit a trade-off, i.e., maximizing rewards (e.g., incompressibility) can degrade fidelity. %Our method aims to achieve a favorable reward-fidelity balance.}

\begin{figure}[t]
    \centering
    \small
    
    \begin{minipage}{0.2\linewidth} \centering Pre-trained \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figures/Original_1x4.png}
    \end{minipage} \vspace{1pt}

    \begin{minipage}{0.2\linewidth} \centering SFT \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figures/SFT_1x4.png}
    \end{minipage} \vspace{1pt}

    \begin{minipage}{0.2\linewidth} \centering RWR \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figures/RWR_1x4.png}
    \end{minipage} \vspace{1pt}

    \begin{minipage}{0.2\linewidth} \centering DPO \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figures/DPO_1x4.png}
    \end{minipage} \vspace{1pt}

    \begin{minipage}{0.2\linewidth} \centering \textbf{Ours} \end{minipage}
    \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figures/Ours_1x4.png}
    \end{minipage}

    \caption{\textbf{Generated samples on the incompressibility task.} While SFT, RWR, and DPO exhibit noticeable structural distortion or severe blurring, our approach (ours) effectively aligns with the target reward without compromising the visual integrity of the original images.
    }
    \label{fig:5x4_samples}
    \vspace{-12pt}
\end{figure}

\paragraph{Baselines}
We compare our method with standard fine-tuning approaches commonly used in reward-driven settings: \textit{Supervised Fine-Tuning (SFT)}, \textit{Reward-Weighted Regression (RWR)} \cite{peters2007reinforcement}, and \textit{Direct Preference Optimization (DPO)} \cite{rafailov2023direct}. {Our goal is to conduct reward-guided fine-tuning on one-step generative models.} To this end, for fair comparison, we transform the multi-step designs of these methods into a single MeanFlow step via single noise injection \cite{FlowGRPO} as
\begin{itemize}[leftmargin=*, topsep=-1pt, itemsep=-1pt]
    % \item \textbf{Supervised Fine-Tuning (SFT)} filters the generated samples to select the highest-reward trajectory within each batch and optimizes selects the highest-reward sample from each batch and fine-tunes the model to reconstruct these optimal samples.
    \item  {\textbf{Supervised Fine-Tuning (SFT)} selects the highest-reward samples within each batch and fine-tunes the model to reconstruct these optimal samples.}
    % \item \textbf{Reward-Weighted Regression (RWR)} frames the problem as reward-weighted likelihood maximization, assigning exponentially higher weights to samples with greater rewards during training.
    \item {\textbf{Reward-Weighted Regression (RWR)} reweights the regression loss by exponentiated rewards.}
    \item \textbf{Direct Preference Optimization (DPO)} leverages a contrastive approach, directly optimizing the policy to increase the likelihood of higher-reward samples over lower-reward ones without requiring an explicit reward model.
\end{itemize}
Detailed formulations and objective functions for each baseline are provided in Appendix \ref{app:imple_details}.

\begin{figure*}[h]
    \centering
    \small

    \begin{subfigure}{0.37\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/off_incomp_reward_plot.pdf}
        \caption{Reward Trajectories.}
        \label{fig:off_incomp_reward}
    \end{subfigure}
    \quad
    \begin{subfigure}{0.37\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/app_samples/incompressibility_reward_fid_xy_plot.pdf}
        \caption{Reward–FID trade-off comparison.}
        \label{fig:incomp_xy}
    \end{subfigure}

    \caption{\textbf{Training dynamics and trade-off analysis on the offline incompressibility task.} The left plot shows reward trajectories during training, while the right plot evaluates the reward–FID trade-off, demonstrating that our method achieves both stable optimization and superior sample quality. For our method, the red diamond marker denotes the reward and FID values at 5,000 steps.}
    \label{fig:off_incomp_combined}
    \vspace{-8pt}
\end{figure*}


\subsection{2D Synthetic Data} \label{sec:2d_synthetic}

To investigate the training dynamics of reward-guided fine-tuning for one-step generators, we conduct a qualitative evaluation using 2D synthetic data. Specifically, a pre-trained model on a standard Gaussian distribution is fine-tuned to target an 8-Gaussian mixture distribution driven by a multi-modal reward signal.

As illustrated in Figure~\ref{fig:2d_8gaussian}, our proposed method exhibits a stable and gradual training dynamic. Throughout the training progression (from 5k to 25k iterations), our approach robustly avoids structural collapse and progressively separates the distribution to capture all eight distinct target modes with high precision. 

In contrast, the baseline methods (SFT, RWR, DPO) struggle to navigate the complex multi-modal reward landscape. As shown in the bottom row of Figure~\ref{fig:2d_8gaussian}, they typically suffer from severe mode averaging, i.e., converging into a continuous ring connecting the targets, or fail entirely to capture the distinct modes. This highlights the effectiveness of our {WGF formulation (\cref{sec:formulation})} in stably guiding the one-step generation process under complex reward signals.




\subsection{Non-Differentiable Reward Optimization} \label{sec:non_diff}
\begin{figure*}[htbp]
    \centering

    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/D_reward.png}
        \caption{Dog Reward Trajectories
        % Our method achieves the highest reward compared to baseline models. DPO is excluded because it is not working in this reward. See Appendix~\ref{tab:reward_DB}
        }
        \label{fig4_reward}
    \end{subfigure}%
    \quad
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/D_fid.png}
        \caption{FID (Dog Subset) Trajectories}
    \end{subfigure}
    
    \caption{\textbf{Reward and FID trajectories for the single-reward dog classification task (Class 5)}. (a) Dog reward trajectories show that our method (red) achieves the highest reward score compared to all baselines. (b) FID computed against the dog subset of CIFAR-10 demonstrates that our method maintains the lowest FID while maximizing reward, confirming effective distribution shift toward the target class without quality degradation. Our method begins at step 2,000 after discriminator warm-up. 
    % Red: Ours, Blue: SFT, Green: RWR, Purple: DPO.
    % \textbf{FID trajectories in the offline dog sampling task in Class 5.} WGF starts at step 2,000 because it warms up updating the Discriminator until then. \textbf{Red}: WGF, \textbf{Blue}: SFT, \textbf{Green}: RWR, \textbf{Purple}: DPO 
    }
    \label{fig: fid_dog}
    \vspace{-8pt}
\end{figure*}

{Our approach does not require gradients of the reward function (\cref{eq:final_objective}), enabling direct application to non-differentiable reward functions. We evaluate our approach on non-differentiable reward tasks: \textit{image compression} and \textit{incompression} defined from \citet{DDPO}.}
% To demonstrate the generalization ability of our approach under complex constraints, we evaluate its performance on non-differentiable reward tasks: image compression and incompression defined from \citet{DDPO}. 
Incompressibility is defined as the file size (KB) of the generated image when saved in JPEG format, encouraging the model to synthesize complex, high-frequency details. Conversely, compressibility is formulated as the negative of the JPEG file size. Because the JPEG compression algorithm is a discrete, black-box operation, these rewards are strictly non-differentiable, making standard gradient-based optimization inapplicable.

% \jw{그러해서 non-differentiable 하다.}



% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/off_incomp_reward_plot.pdf}
%     \caption{Reward trajectories on the offline incompressibility task. Our method achieves more stable and consistently higher reward optimization compared to SFT, RWR, and DPO. 
%     % \jw{이게 RWR 수정한 버전의 실험 결과인가요?}
%     % } \woorim{RWR 수정하기 전 버전의 실험 결과인데, 수정 후 버전도 이 라인 플랏과 유사하게 5000 스텝에서 1.09 정도로 마무리되는 양상을 보입니다 ... (수정 전 버전과 크게 달라진 점이 없음)
%     }
%     \label{fig:off_incomp_reward_plot}
% \end{figure}




% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/app_samples/incompressibility_reward_fid_xy_plot.pdf}
%     % \caption{Reward-FID trade-off comparison under the incompressibility reward.}
%     \caption{Comparison of incompressibility reward-FID trade-off across methods.}
%     \label{fig:incomp_xy}
% \end{figure}


% \woorim{figure 2, 4를 subfigure로?}


\paragraph{Incompression}
% \jw{Reward + FID figure 나오면 수정. Figure ?? shows how the reward and FID changes throughout the training process. ---. Figure ?? presents the qualitative results. ---}

In the incompression task, baselines struggle to optimize the reward without compromising structural integrity (see Figure~\ref{fig:5x4_samples}). As shown in Figure~\ref{fig:off_incomp_reward}, SFT and RWR do not improve the reward, even decreasing from the initial value of approximately 1.29, and generate progressively blurrier samples. This indicates that the optimization dynamics inherited from likelihood-based fine-tuning dominate the reward signal. While DPO achieves quantitative improvements, the resulting images are severely corrupted by noise and blurring artifacts, which significantly degrades the overall perceptual quality.

% Figure~\ref{fig:incomp_xy} further illustrates the relationship between reward and FID across all methods. It reveals that baselines either fail to meaningfully optimize the reward (SFT, RWR) or suffer from perceptual degradation when slight reward improvements are made (DPO). In contrast, our method achieves a highly favorable trade-off, simultaneously maintaining higher reward while keeping FID stable, demonstrating more effective optimization in the incompressibility task.

Figure~\ref{fig:incomp_xy} further illustrates the relationship between reward and FID across all methods. It reveals that baselines struggle with effective optimization in different ways: SFT fails to meaningfully improve the reward, RWR suffers from a severe collapse in image quality without any reward gain, and DPO exhibits perceptual degradation when slight reward improvements are made. In contrast, our method achieves a highly favorable trade-off, simultaneously maintaining a higher reward while keeping the FID stable, demonstrating more effective optimization in the incompressibility task.


Figure~\ref{fig:5x4_samples} presents qualitative results. Our method effectively injects high-frequency details to maximize the incompressibility reward while preserving the semantic structures of the original images. Similar patterns of optimization failure and severe blurring in baselines are consistently observed in the compressibility task (additional results are provided in Appendix~\cref{app:non_diff}).

% \paragraph{Comparison of Multi-Step Generator}
\paragraph{Comparison with Multi-Step Methods}
{
While reward-guided fine-tuning of multi-step diffusion models has been actively investigated \citep{DPOK, DDPO, gao2025reward}, fine-tuning methods specifically designed for one-step generators remain largely unexplored. 
% To our knowledge, our work represents the first principled approach to this problem. 
To contextualize the effectiveness of our method, we provide a relative comparison against these multi-step approaches, despite the fundamental differences in problem setting and network architecture.
}

{Table~\ref{tab:merged_comparison} compares our one-step approach against multi-step fine-tuning methods from \citet{gao2025reward}, which use q-Learning and DPOK on a pretrained DDPM with 20 sampling steps. Note that the restricted 20 sampling steps (reduced from 1000 in the original setup \citep{denoising}). Their setup starts at reward 1.10 and FID 29.90. Our pretrained MeanFlow model, designed for one-step generation, starts at reward 1.29 and FID 3.90. Despite being the first method tailored for one-step fine-tuning and requiring only a single network evaluation (vs. 20), our approach achieves superior reward-FID trade-offs. 
% By adjusting the parameter $\beta$, our approach successfully increases the target reward while maintaining a significantly lower FID, demonstrating stable optimization even at one sampling step.
}
 
% We further compare the trade-off between reward and FID on the incompressibility task against the multi-step reward-guided fine-tuning approach. The performance results for the baseline algorithms (q-Learning and DPOK) are directly reported from \citet{gao2025reward}. To ensure a rigorous and fair comparison, we compute the FID against the full CIFAR-10 training set, strictly adhering to their evaluation protocol. As shown in Table~\ref{tab:merged_comparison}, \citet{gao2025reward} uses a pre-trained DDPM (Initial Reward: 1.10, FID: 29.90) which is restricted to a reduced number of sampling steps ($K=20$) due to computational costs. Consequently, their baseline model suffers from severe degradation in sample quality, driving a significantly high FID. 

% In contrast, our proposed method, which leverages a one-step pre-trained MeanFlow model from \citet{MeanFlow} (Initial Reward: 1.29, FID: 3.90), achieves a superior trade-off. By adjusting the parameter $\beta$, our approach successfully increases the target reward while maintaining a significantly lower FID, demonstrating stable optimization even at one sampling step.

% \begin{table}[htbp]
%     \centering
%     \caption{Performance comparison of reward-guided fine-tuning methods. Multi-step baseline results are adopted from \cite{gao2025reward}.
%     \jw{pretrained model이 DDPM과 meanflow로 다르다는걸 표에 추가해주세요.}
%     }
%     \label{tab:merged_comparison}
%     \begin{tabular}{clcc}
%         \toprule
%         \multicolumn{2}{c}{Algorithm} & Reward (KB) $\uparrow$ & FID $\downarrow$ \\
%         \midrule[0.8pt]
%         \multicolumn{4}{l}{Pre-trained DDPM} \\
%         \midrule
%         \multicolumn{2}{c}{q-Learning} & \multirow{2}{*}{1.20} & 26.64 \\
%         \multicolumn{2}{c}{DPOK} & & 77.94 \\
%         \midrule
%         \multicolumn{2}{c}{q-Learning} & \multirow{2}{*}{1.30} & 50.58 \\
%         \multicolumn{2}{c}{DPOK} & & 107.99 \\
%         \midrule
%         \multicolumn{2}{c}{q-Learning} & \multirow{2}{*}{1.40} & 89.79 \\
%         \multicolumn{2}{c}{DPOK} & & 138.89 \\
%         \midrule[0.8pt]
%         \multicolumn{4}{l}{Pre-trained MeanFlow} \\
%         \midrule
%         \multirow{3}{*}{Ours} & $\beta = 1$ & 1.33 & 5.43 \\
%          & $\beta = 3$ & 1.42 & 9.32 \\
%          & $\beta = 5$ & 1.53 & 24.99 \\
%         \bottomrule
%     \end{tabular}
%     % \caption{Performance comparison of reward-guided fine-tuning methods. Note that the baselines (q-Learning, DPOK) from \cite{gao2025reward} are fine-tuned from a pre-trained DDPM (Initial Reward: 1.10, FID: 29.90), whereas our proposed method is based on MeanFlow (Initial Reward: 1.29, FID: 3.90). Our method achieves competitive rewards while better preserving image quality. \jw{q-learning과 DPOK 결과는 기존 논문에서 가져왔다고 explicit하게 적기. 캡션이 좀 길어서 initial model 관련 내용은 캡션에서 빼고 본문으로}
%     % }
    
% \end{table}

\begin{table}[htbp]
    \centering
    \caption{\textbf{Performance comparison of reward-guided fine-tuning methods.} Multi-step baseline results are adopted from q-Learning \cite{gao2025reward}.}
    \label{tab:merged_comparison}
    \scalebox{0.9}{
    \begin{tabular}{clccc}
        \toprule
        Model & \multicolumn{2}{c}{Algorithm} & Reward (KB) $\uparrow$ & FID $\downarrow$ \\
        \midrule
        \multirow{6}{*}{DDPM}
        & \multicolumn{2}{c}{q-Learning} & \multirow{2}{*}{1.20} & 26.64 \\
        & \multicolumn{2}{c}{DPOK}       &                       & 77.94 \\
        \cmidrule(lr){2-5}
        & \multicolumn{2}{c}{q-Learning} & \multirow{2}{*}{1.30} & 50.58 \\
        & \multicolumn{2}{c}{DPOK}       &                       & 107.99 \\
        \cmidrule(lr){2-5}
        & \multicolumn{2}{c}{q-Learning} & \multirow{2}{*}{1.40} & 89.79 \\
        & \multicolumn{2}{c}{DPOK}       &                       & 138.89 \\
        \midrule
        \multirow{3}{*}{MeanFlow}
        & \multirow{3}{*}{Ours} & $\beta = 1$ & 1.33 & 5.43 \\
        &                       & $\beta = 3$ & 1.42 & 9.32 \\
        &                       & $\beta = 5$ & 1.53 & 24.99 \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{-8pt}
\end{table}

% \subsection{Differentiable and Explicitly defined Reward} 
\subsection{Differentiable Reward Optimization} 
\label{sec:diff}
We now evaluate our method on CIFAR-10 under two differentiable reward configurations: (1) a single-reward setting and (2) a multiple-reward setting. {Here, we consider two reward functions: the class probability for the dog class (class 5) and the image brightness. We report the reward score and FID computed against the \textit{dog class} of CIFAR-10.}

% We report the class-targeted reward score and FID \cite{NIPS2017_8a1d6947}, which reflect complementary aspects of reward fine-tuning. \jin{수정된 5.1이랑 중복됨}The reward score directly evaluates the effectiveness of reward-guided fine-tuning, assessing whether the generator distribution has shifted toward the high-reward target. The FID evaluates whether the model retains the fidelity of the pretrained distribution without collapsing into reward hacking. To explicitly verify this targeted distribution shift, we measure the class-wise FID specifically against the subset of the target class.

% \jw{각 metric이 평가하는 attribute 설명. final reward는 reward-guided fine-tuning 평가. FID는 reward-hacking이 발생하지 않고 fidelity 유지하는지 평가. 각 metric에 cite}
% \jw{FID 샘플 갯수 같은 디테일은 appendix}
% \js{지금은 실험이 많지않아서 그렇지만, 이런 metric은 모든 실험에 반복적으로 사용되므로 5.1로 옮겨두는 것이 좋음. 최재웅 교수님말처럼 기계적으로다른 논문 구조 모방해도됨.}

\paragraph{Single Classification Reward} 
% In this section, we demonstrate the result of testing the single classification reward: class 5 (dog) in CIFAR-10. Specifically, given a pretrained ResNet-56 classifier $f_\phi: \mathbb{R}^{3\times 32\times 32} \to \mathbb{R}^{10}$ and the input normalization $N(\cdot)$ used during classifier training, the reward for the dog class (class 5) is defined as:
In this section, we demonstrate the result of testing the single classification reward: class 5 (dog) in CIFAR-10. Specifically, given a pretrained ResNet-56 classifier $p_\phi: \mathbb{R}^{3\times 32\times 32} \to \mathbb{R}^{10}$, the reward is defined as $r(y) = \log p_\phi\big(c = 5 \,\big|\, y\big)$.

% \begin{equation}
% \begin{split}
% R(y) &= \log p_\phi\big(c = 5 \,\big|\, N(y)\big) \\
%      &= \log \text{softmax}\big(f_\phi(N(y))\big)_5
% \end{split}
% \end{equation}
% \begin{equation}
% r(y) = \log p_\phi\big(c = 5 \,\big|\, y\big)
% \end{equation}

Figure~\ref{fig: fid_dog} compares the reward scores across methods. Our method attains the highest reward score ($\approx-0.87$) among all methods. {FID compared to the dog subset of CIFAR-10 is significantly smaller than baselines. This confirms that meaningful alignment has occurred in our model, well-reward-guided and not escaped from the original targeted distribution, the dog set of CIFAR-10. In contrast, the baseline methods (SFT, RWR, and DPO) show minimal reward improvement, indicating unsuccessful optimization.

% Although our model reports a high FID calculated with the full CIFAR-10, FID compared to the dog subset of CIFAR-10 is significantly smaller than baselines (see Appendix \ref{fig_2(2)}). This confirms that meaningful alignment has occurred in our model, well-reward-guided and not escaped from the original targeted distribution, the Dog set of Cifar-10.

\begin{figure*}[htbp]
    \centering

    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/DB_reward.png}
        \caption{Dog and Bright Reward Trajectories
        }
        % Dog and Bright Reward trajectories. Our method achieves the highest reward compared to baseline models. DPO is excluded because it is not working in this reward. See Appendix~\ref{tab:reward_DB}}
        \label{fig4_reward}
    \end{subfigure}%
    \quad
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/DB_fid.png}
        \caption{FID (Dog Subset)}
    \end{subfigure}
    
    % \caption{FID trajectories in the offline dog sampling task in Dog and Brightness. WGF starts at step 2000 because it warms up updating the Discriminator until then. \textbf{Red}: WGF, \textbf{Blue}: SFT, \textbf{Green}: RWR, \textbf{Purple}: DPO.}
    \caption{\textbf{Reward and FID trajectories for multi-reward optimization (dog classification + brightness).} (a) Combined reward trajectories show that our method (red) achieves the highest reward score, successfully optimizing both objectives simultaneously. 
    % Baselines struggle to balance multiple rewards, showing minimal improvement (SFT, blue) or stagnation (RWR, green; DPO, purple). 
    (b) FID computed against the dog subset demonstrates that our method maintains the lowest FID while maximizing rewards, confirming effective multi-objective alignment without quality degradation. 
    % Our method begins at step 2,000 after discriminator warm-up. 
    % \textbf{Red}: Ours, \textbf{Blue}: SFT, \textbf{Green}: RWR, \textbf{Purple}: DPO.
    }
    \label{fig: fid_dog_bright}
    % \vspace{-8pt}
\end{figure*}


\begin{figure*}[h]
    \centering

    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/incompressibility_ours_beta_plot.pdf}
        \caption{Reward Trajectory}
        \label{fig:reward_beta}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/incompressibility_ours_beta_fid_plot.pdf}
        \caption{FID Trajectory}
        \label{fig:fid_beta}
    \end{subfigure}
    
    \caption{{Effect of $\beta$ on Incompressibility Reward and image quality (FID).}}
    % \vspace{-8pt}
    \label{fig:overall_beta_effect}
\end{figure*}

\paragraph{Multi-Reward} 
{We evaluate on a multi-reward setting by combining class 5 probability and image brightness, following \cite{FlowGRPO}.}
% We also evaluated the models in a multi-reward setting following the multi-reward composition in \cite{FlowGRPO}. Instead of PickScore or OCR, Class 5 of CIFAR-10 (dog) and brightness are our targets. 
Let $x \in [-1, 1]^{3\times32\times32}$ be the generated image tensor and $c$ be the target class index. We define the brightness score $\mathcal{B}(x)$ as the normalized average of the pixel values, i.e., $\mathcal{B}(x) = \frac{1}{N} \sum_{i=1}^{N} \frac{x_i + 1}{2}$.
% \begin{equation}
%     \mathcal{B}(x) = \frac{1}{N} \sum_{i=1}^{N} \frac{x_i + 1}{2}
% \end{equation}
where $N$ is the total number of pixels in the image tensor. Let $P(y=c|x)$ denote the probability of the image $x$ belonging to class $c$, as predicted by a pre-trained classifier. {The combined reward is:}
% Eq \eqref{eq:ours} and Eq \eqref{eq:baseline} indicate the formulation of rewards.
% \begin{equation}
% \label{eq:ours}
% \begin{aligned}
%     R_{\text{ours}}(x) = \max \Big( & w_{\text{dog}} \cdot P(y=c|x) \\
%     & + w_{\text{bright}} \cdot \mathcal{B}(x), 10^{-6} \Big)
% \end{aligned}
% \end{equation}
% \begin{equation}
% \label{eq:baseline}
% \begin{aligned}
%     R_{\text{baseline}}(x) = & \; w_{\text{dog}} \cdot \log \big( \max(P(y=c|x), 10^{-4}) \big) \\
%     & + w_{\text{bright}} \cdot \max(\mathcal{B}(x), 10^{-4})
% \end{aligned}
% \end{equation}
\begin{align}
\small
R_{\text{ours}}(x)
&= \max \Big(
    w_{\text{dog}} \cdot P(y=c|x) \notag \\
&\qquad\qquad
    + w_{\text{bright}} \cdot \mathcal{B}(x), 10^{-6}
\Big)
\label{eq:ours} \\
R_{\text{baseline}}(x)
&= w_{\text{dog}} \cdot \log \big( \max(P(y=c|x), 10^{-4}) \big) \notag \\
&\qquad
    + w_{\text{bright}} \cdot \max(\mathcal{B}(x), 10^{-4})
\label{eq:baseline}
\end{align}


Figure~\ref{fig: fid_dog_bright} illustrates the computed reward scores, identical to the single-reward evaluation. WGF significantly outperforms all baselines in the reward score across training.

Additionally, the advantage of WGF extends to balancing multiple rewards since the baselines are poor at it or even show decreases when they are asked to increase the multiple rewards; dog score and brightness.


\subsection{Ablation Study} \label{sec:ablation_study}
% As illustrated in Figure~\ref{fig:overall_beta_effect}, we conduct an ablation study on the parameter $\beta$, which determines the weight of the target reward during the optimization process. 
We conduct an ablation study on the parameter $\beta$, which determines the weight of the target reward during the optimization process.
Figure~\ref{fig:overall_beta_effect} shows the reward and FID trajectories for the incompressibility task across different $\beta$.
As $\beta$ increases, we observe a proportional and stable rise in the achieved reward, demonstrating robust controllability over the generative objective. Correspondingly, FID increases, reflecting the expected reward-fidelity trade-off. Even at $\beta=20$, the model maintains reasonable proximity to the pretrained data manifold, showing that our method effectively prevents catastrophic reward hacking.
% Although optimizing for higher rewards inherently increases the FID, we observe that this quality degradation is strictly constrained. Despite the strong optimization pressure at high $\beta$ values ($\beta \in [1, 20]$), the model effectively resists arbitrary distribution shifts and maintains reasonable proximity to the pretrained data manifold. By doing so, our approach reliably maximizes the target reward while preventing catastrophic reward hacking, confirming its robustness across diverse hyperparameter settings.


\section{Conclusion}
In this paper, we propose the first reward-guided fine-tuning framework for one-step generative models via Wasserstein Gradient Flow (WGF). Existing methods designed for multi-step diffusion models cannot be directly applied to one-step generators due to the absence of iterative denoising steps. Our approach formulates fine-tuning as a WGF problem, which is discretized through the JKO scheme.
Our method enables stable distributional updates that mitigate reward hacking, handles non-differentiable rewards, and provides controllable reward-fidelity trade-offs. Experiments demonstrate superior performance on both synthetic and real datasets compared to baseline approaches, establishing a principled foundation for efficient reward alignment in one-step generative models.

% \clearpage
